A comprehensive study on the relation between the metal enrichment of ionised and atomic gas in star-forming galaxies

We study the relation between the metallicities of ionised and atomic gas in star-forming galaxies at z=0-3 using the EAGLE cosmological, hydrodynamical simulations. This is done by constructing a dense grid of sightlines through the simulated galaxies and obtaining the star formation rate- and HI column density-weighted metallicities, Z_{SFR} and Z_{HI}, for each sightline as proxies for the metallicities of ionised and atomic gas, respectively. We find Z_{SFR} > Z_{HI} for almost all sightlines, with their difference generally increasing with decreasing metallicity. The stellar masses of galaxies do not have a significant effect on this trend, but the positions of the sightlines with respect to the galaxy centres play an important role: the difference between the two metallicities decreases when moving towards the galaxy centres, and saturates to a minimum value in the central regions of galaxies, irrespective of redshift and stellar mass. This implies that the mixing of the two gas phases is most efficient in the central regions of galaxies where sightlines generally have high column densities of HI. However, a high HI column density alone doesn't guarantee a small difference between the two metallicities. In galaxy outskirts, the inefficiency of the mixing of star-forming gas with HI seems to dominate over the dilution of heavy elements in HI through mixing with the pristine gas. We find good agreement between the available observational data and the Z_{SFR}-Z_{HI} relation predicted by the EAGLE simulations. Though, observed regions with a nuclear-starburst mode of star formation appear not to follow the same relation.

==> abstract <==
We study the relation between the metallicities of ionised and atomic gas in star-forming galaxies at z=0-3 using the EAGLE cosmological, hydrodynamical simulations. This is done by constructing a dense grid of sightlines through the simulated galaxies and obtaining the star formation rate- and HI column density-weighted metallicities, ZSFR and ZHI, for each sightline as proxies for the metallicities of ionised and atomic gas, respectively. We find ZSFR \gtrsim ZHI for almost all sightlines, with their difference generally increasing with decreasing metallicity. The stellar masses of galaxies do not have a significant effect on this trend, but the positions of the sightlines with respect to the galaxy centres play an important role: the difference between the two metallicities decreases when moving towards the galaxy centres, and saturates to a minimum value in the central regions of galaxies, irrespective of redshift and stellar mass. This implies that the mixing of the two gas phases is most efficient in the central regions of galaxies where sightlines generally have high column densities of HI. However, a high HI column density alone doesn't guarantee a small difference between the two metallicities. In galaxy outskirts, the inefficiency of the mixing of star-forming gas with HI seems to dominate over the dilution of heavy elements in HI through mixing with the pristine gas. We find good agreement between the available observational data and the ZSFR-ZHI relation predicted by the EAGLE simulations. Though, observed regions with a nuclear-starburst mode of star formation appear not to follow the same relation. 

